Neural Contractive Dynamical Systems

Stability guarantees are crucial when ensuring a fully autonomous robot does not take undesirable or potentially harmful actions. Unfortunately, global stability guarantees are hard to provide in dynamical systems learned from data, especially when the learned dynamics are governed by neural networks. We propose a novel methodology to learn neural contractive dynamical systems, where our neural architecture ensures contraction, and hence, global stability. To efficiently scale the method to high-dimensional dynamical systems, we develop a variant of the variational autoencoder that learns dynamics in a low-dimensional latent representation space while retaining contractive stability after decoding. We further extend our approach to learning contractive systems on the Lie group of rotations to account for full-pose end-effector dynamic motions. The result is the first highly flexible learning architecture that provides contractive stability guarantees with capability to perform obstacle avoidance. Empirically, we demonstrate that our approach encodes the desired dynamics more accurately than the current state-of-the-art, which provides less strong stability guarantees.

==> Sections/Results/Comparison.tex <==
    \subsection*{Comparisons}
    
    To perform comparison between different approaches, we have constructed a synthetic dataset by combining various LASA datasets.

    \begin{equation}
        \mathcal{D} = [ x_{Angle}, y_{Angle}, x_{Line}, y_{Line}, x_{Sine}, y_{Sine}, x_{JShape}, y_{JShape} ] \in \mathbb{R} ^ {T \times 8}
    \end{equation}
    
    Figure~\ref{fig:dtwd} illustrates the average time warping distance across five distinct path integrals generated using each respective method and all the available demonstrations. As this figure shows NCDS has the highest accuracy in reproducing motion trajectories similar to the provided demonstrations. Based on this comparison, SEDS shows better reconstruction than EF and IF. For completeness, Figure~\ref{fig:traj_comparison} shows the generated path integrals. Evidently, our approach exhibits the highest reconstruction accuracy. 

    \textbf{Experimental setups:}
    \begin{itemize}
        \item \textbf{Imitation Flow}: For Imitation Flow we have used a imitation flow network with the depth of $10$. Each level within this depth was  constructed utilizing CouplingLayer, RandomPermutation, and LULinear techniques, as recommended by the authors for managing high-dimensional data. The training process includes $1000$ epochs, with a empirically chosen learning rate of $10^{-3}$. These hyper parameters were found experimentally and the best results have been selected to be compared against. 
        \item \textbf{Euclidenizing Flow}: Here, we have used coupling network with random Fourier features parameterization, with 10 coupling layers each with 200 hidden units, and length scale of $0.45$ as the length scale for random Fourier features. The training process includes $1000$ epochs, with a empirically chosen learning rate of $10^{-4}$. These hyper parameters were found experimentally and the best results have been selected to be compared against.
        \item \textbf{SEDS}: Here, we use $10$ Gaussian functions. The training process includes $1000$ epochs with MSE objective.
    \end{itemize}
    
    \begin{figure}[h!]
        \centering
            \includegraphics[width=0.5\textwidth]{Images/Comparisons/DTWD.pdf}
            \caption{Average dynamic time warping distance between 5 trajectories constructed with different methods and demonstration trajectories}
            \label{fig:dtwd}
    \end{figure}

        \begin{figure}[h!]
        \begin{center}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/ncds_traj0.pdf}
    \end{subfigure}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/ef_traj0.pdf}
    \end{subfigure}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/if_traj0.pdf}
    \end{subfigure}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/seds_traj0.pdf}
    \end{subfigure}\\
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/ncds_traj1.pdf}
    \end{subfigure}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/ef_traj1.pdf}
    \end{subfigure}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/if_traj1.pdf}
    \end{subfigure}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/seds_traj1.pdf}
    \end{subfigure}\\
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/ncds_traj2.pdf}
    \end{subfigure}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/ef_traj2.pdf}
    \end{subfigure}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/if_traj2.pdf}
    \end{subfigure}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/seds_traj2.pdf}
    \end{subfigure}\\
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/ncds_traj3.pdf}
        \caption{NCDS}
    \end{subfigure}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/ef_traj3.pdf}
        \caption{EF}
    \end{subfigure}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/if_traj3.pdf}
        \caption{IF}
    \end{subfigure}
    \begin{subfigure}{0.17\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/seds_traj3.pdf}
        \caption{SEDS}
    \end{subfigure}
    \caption{Path integrals generated using different methods. }
    \label{fig:traj_comparison}
    \end{center}
    \end{figure}



==> Sections/Results/Quan_results.tex <==
    \subsection*{Quantitative results}
    
    \textbf{Regularization}: It is imperative to clarify that the regularization term, known as epsilon $\epsilon$, plays a crucial role in defining the upper bound for the eigenvalues of the Jacobian, which inherently governs the contraction rate of the system. Figure~\ref{fig:traj_epsilon} illustrates the effect of $\epsilon$ on the accuracy of the system. Adjusting this value, particularly through increments, has the potential to detrimentally affect the network's expressiveness, therefore compromising the reconstruction process.

    \noindent
    The observed negative effect can be attributed to the fact that this regularization is applied to the entire Jacobian matrix and not exclusively to the elements responsible for preserving the negative definiteness of the Jacobian. As a result, it might inadvertently penalize essential components of the Jacobian, leading to adverse consequences on the model's expressivity. A more targeted approach that focuses solely on the relevant elements could potentially mitigate these undesired effects and enhance the regularization's overall effectiveness.
    \begin{figure}
        \begin{center}
            \begin{subfigure}{0.2\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Images/Angle_evolution_1e-4.pdf}
                \caption{$\epsilon = 10^{-4}$}
            \end{subfigure}
            \begin{subfigure}{0.2\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Images/Angle_evolution_1e-2.pdf}
                \caption{$\epsilon = 10^{-2}$}
            \end{subfigure}
            \begin{subfigure}{0.2\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Images/Angle_evolution_1e-1.pdf}
                \caption{$\epsilon = 10^{-1}$}
            \end{subfigure}
            \begin{subfigure}{0.2\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Images/Angle_evolution_10.pdf}
                \caption{$\epsilon = 10$}
            \end{subfigure}
            \caption{Velocity profile over time in a single path integral}
            \label{fig:traj_epsilon}
        \end{center}
    \end{figure}

    \noindent
    \textbf{Integration}: Furthermore, we have tested the integrator in a toy example constructed using a Sine wave under different conditions. Figure~\ref{fig:vel_int_step} shows the integrator under different conditions. Figure~\ref{fig:vel_int_step}-a and -b: when the absolute and relative tolerance parameters of the integrator need to be at least as $10^{-3}$. Figure~\ref{fig:vel_int_step}-c shows that the number of time steps to solve the integration does not make any difference. Furthermore, Figure~\ref{fig:vel_int_step}-d displays different integration methods and their data reconstruction accuracy.

    \begin{figure}[h!]
    \begin{center}
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/Sine_wave_different_atol.pdf}
        \caption{Comparison among different absolute tolerance values}
    \end{subfigure}%
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/Sine_wave_different_rtol.pdf}
        \caption{Comparison among different relative tolerance values}
    \end{subfigure}\\
        \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/Sine_wave_different_t.pdf}
        \caption{Comparison among different integration time steps}
    \end{subfigure}%
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Comparisons/Sine_wave_different_integrtors.pdf}   
        \caption{Comparison among different integration methods}
    \end{subfigure}
    \caption{Evaluation of the integrator}
    \label{fig:vel_int_step}
        \end{center}
\end{figure}

    \noindent
    \textbf{Activation function}: The choice of activation function certainly effects the generalization in the dynamical system (where there is no data). To show this phenomena, we have ablated few activation functions. For this experimental setup, we employed a feedforward neural network comprising two hidden layers, each consisting of $100$ units. 

    \noindent
    As shown in Figure~\ref{fig:activation_function}, both the \textit{Tanh} and \textit{Softplus} activation functions display superior performance, coupled with satisfactory generalization capabilities. This indicates that the contour of the vector field aligns with the overall demonstration behavior outside of the data support. Conversely, opting for the Sigmoid activation function might yield commendable generalization beyond the confines of the data support. However, it is essential to acknowledge that this choice could potentially encounter challenges when it comes to reaching and stopping at the target.
    
    \begin{figure}[h!]
    \begin{center}
    \begin{subfigure}{0.20\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Angle_evolution_1e-4.pdf}
        \caption{Tanh}
    \end{subfigure}%
    \begin{subfigure}{0.20\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Angle_evolution_1e-4_softplus.pdf}
        \caption{Softplus}
    \end{subfigure}
        \begin{subfigure}{0.20\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/Angle_evolution_1e-4_Sigmoid.pdf}
        \caption{Sigmoid}
    \end{subfigure}

    \caption{Velocity profile over time in a single path intergral}
    \label{fig:activation_function}
        \end{center}
\end{figure}

    \noindent
    \textbf{Dimensionality and execution time}: Table 1 compares 4 different experimental setups.  First, Table 1-a reports the average execution time under the setup where the dimensionality reduction (i.e., no VAE) is discarded and the dynamical system is learned directly in the input space. As the table shows, under this setting, increasing the dimensionality of the input space from $2$ to $8$ entails a remarkable $40$-fold increase in execution time for a single integration step. This empirical relationship reaffirms the inherent computational intensity tied to Jacobian-based computations. To address this issue, our approach leverages the dimensionality reduction provided by a custom Variational Autoencoder (VAE) that takes advantage of an injective generator (as decoder) and its inverse (as encoder). As showcased in Table 1-b, the VAE distinctly mitigates the computational burden. Comparing Table 1-a and 1-b, the considerable advantages of integrating the contractive dynamical system with the VAE into the full pipeline become evident as it leads to a significant halving of the execution time in the 8D scenario. 

    \noindent
    Moreover, the presented results indicate that our current system may not achieve real-time operation. However, it is noteworthy that the new video footage from our real-world robot experiments convincingly demonstrates the system's rapid query response time, sufficiently efficient to control the robot arm, devoid of any operational concerns.
    % \textbf{Learning}: 
    % % mention the learning rate 
    % % mention the architecture 
    % % the loss 
    % \begin{figure}[h!]
    %     \centering
    %         \includegraphics[width=0.5\textwidth]{Images/loss.png}
    %         \caption{}
    %         \label{fig:loss}
    % \end{figure}    

    
